SMACE: A New Method for the Interpretability of Composite Decision Systems

Interpretability is a pressing issue for decision systems. Many post hoc methods have been proposed to explain the predictions of a single machine learning model. However, business processes and decision systems are rarely centered around a unique model. These systems combine multiple models that produce key predictions, and then apply decision rules to generate the final decision. To explain such decisions, we propose the Semi-Model-Agnostic Contextual Explainer (SMACE), a new interpretability method that combines a geometric approach for decision rules with existing interpretability methods for machine learning models to generate an intuitive feature ranking tailored to the end user. We show that established model-agnostic approaches produce poor results on tabular data in this setting, in particular giving the same importance to several features, whereas SMACE can rank them in a meaningful way.

==> eval/linearmodels/case_paper_rule.tex <==
\begin{table}
\caption{\label{tab:paper_rule}Simple hybdrid system, explaining the rule-based decision.
$x_1$ is very close to the decision boundary: $r_1$ is very high, while $r_4=0$ since $x_4$ is not directly involved within the decision policy.}
    \centering
    \begin{tabular}{l l | r}
    condition & $\xi^{(1)}$ & $r$ \\
    \hline
    $x_1\leq0.5$ & $0.6$ & $-0.90$ \\
    $x_2\geq0.6$ & $0.1$ & $-0.50$ \\
    $x_3$ & $0.4$ & $0.00$  \\
    $m_1\geq1$ & $0.6$ & $-0.87$ \\
    $m_2\leq600$ & $320$ & $0.86$ \\
    \end{tabular}
\end{table}


==> tikz/trace.tex <==
%\centering

\forestset{
    trace/.style={edge+={color=blue,line width=1.5pt}},
}

\begin{forest}
[$x_1\geq 0.5$, trace, color=blue, tikz={\draw[{Latex}-, thick] (.north) --++ (0,0.6);}
    [$x_2\geq 0.7$
        [4]
        [3]    
    ]
    [$x_2\geq 0.3$, trace, color=blue
        [2]   
        [1, trace, color=blue] 
    ]   
] 
\end{forest}
